Systems of random linear equations and the phase transition in MacArthur's resource-competition model

Complex ecosystems generally consist of a large number of different species utilizing a large number of different resources. Several of their features cannot be captured by models comprising just a few species and resources. Recently, Tikhonov and Monasson have shown that a high-dimensional version of MacArthur's resource competition model exhibits a phase transition from a 'vulnerable' to a 'shielded' phase in which the species collectively protect themselves against an inhomogeneous resource influx from the outside. Here we point out that this transition is more general and may be traced back to the existence of non-negative solutions to large systems of random linear equations. Employing Farkas' Lemma we map this problem to the properties of a fractional volume in high dimensions which we determine using methods from the statistical mechanics of disordered systems.

==> bibliography <==
%Paper ueber die erstaunliche Vielfalt der Arten

@article{hutchinson1959homage,
  title={Homage to Santa Rosalia or why are there so many kinds of animals?},
  author={Hutchinson, G Evelyn},
  journal={The American Naturalist},
  volume={93},
  number={870},
  pages={145--159},
  year={1959},
  publisher={Science Press}
}



%Diversitaet in Regenwaeldern
@book{ghazoul2010tropical,
  title={Tropical rain forest ecology, diversity, and conservation},
  author={Ghazoul, Jaboury and Sheil, Douglascoaut},
  publisher={Oxford University Press},
  year={2010}
}











%Hohe Diversitaet des menschlichen Mikrobioms

@article{lozupone2012diversity,
  title={Diversity, stability and resilience of the human gut microbiota},
  author={Lozupone, Catherine A and Stombaugh, Jesse I and Gordon, Jeffrey I and Jansson, Janet K and Knight, Rob},
  journal={Nature},
  volume={489},
  number={7415},
  pages={220},
  year={2012},
  publisher={Nature Publishing Group}
}
%Main Paper von Tihkonov und Monasson

@article{TM17,
  title = {Collective Phase in Resource Competition in a Highly Diverse Ecosystem},
  author = {Tikhonov, Mikhail and Monasson, Remi},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {4},
  pages = {048103},
  numpages = {5},
  year = {2017},
  month = {1},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.048103},
}


%Folgepaper von Tikhonov und Monasson
@article{tikhonov2017innovation,
  title={Innovation rather than improvement: a solvable high-dimensional model highlights the limitations of scalar fitness},
  author={Tikhonov, Mikhail and Monasson, Remi},
  journal={Journal of Statistical Physics},
  volume={172},
  number={74},
  pages={74},
  year={2018},
  publisher={Springer}
}

%Beispiel an dem Biodiversitaet mit wenigen Spezies untersucht wird
@article{huisman1999biodiversity,
  title={Biodiversity of plankton by species oscillations and chaos},
  author={Huisman, Jef and Weissing, Franz J},
  journal={Nature},
  volume={402},
  number={6760},
  pages={407},
  year={1999},
  publisher={Nature Publishing Group}
}


%Generel Statistische Physik angewandt auf interdisziplinaere Probleme, auch Biodiversitaet
@article{castellano2009statistical,
  title={Statistical physics of social dynamics},
  author={Castellano, Claudio and Fortunato, Santo and Loreto, Vittorio},
  journal={Reviews of modern physics},
  volume={81},
  number={2},
  pages={591},
  year={2009},
  publisher={APS}
}



%Hier kommt das Ursprungsmodell her

@article{macarthur_species_1970,
	title = {Species packing and competitive equilibrium for many species},
	volume = {1},
	doi = {10.1016/0040-5809(70)90039-0},
	number = {1},
	journal = {Theoretical Population Biology},
	author = {MacArthur, Robert},
	month = may,
	year = {1970},
	pages = {1--11},
}



%Arbeit auf der das Tikhonov Monasson Paper beruht

@article{tikhonov2016community,
  title={Community-level cohesion without cooperation},
  author={Tikhonov, Mikhail},
  journal={Elife},
  volume={5},
  year={2016},
  publisher={eLife Sciences Publications, Ltd}
}


%Tilman hat das Ursprungsmodell zum ersten Mal richtig untersucht

@book{tilman1982resource,
  title={Resource competition and community structure},
  author={Tilman, David},
  year={1982},
  publisher={Princeton University Press}
}


%Hier wird das MacArthur Modell mit dem Cavity approach untersucht

@article{advani2017environmental,
  title={Environmental engineering is an emergent feature of diverse ecosystems and drives community structure},
  author={Advani, Madhu and Bunin, Guy and Mehta, Pankaj},
  journal={arXiv preprint arXiv:1707.03957},
  year={2017}
}


%Hier werden zufaellige Lotka-Volterra Gleichungen mit Replika untersucht

@article{biroli2017marginally,
  title={Marginally Stable Equilibria in Critical Ecosystems},
  author={Biroli, Giulio and Bunin, Guy and Cammarota, Chiara},
  journal={arXiv preprint arXiv:1710.03606},
  year={2017}
}


%Review of MacArthur Model

@article{chesson1990macarthur,
  title={MacArthur's consumer-resource model},
  author={Chesson, Peter},
  journal={Theoretical Population Biology},
  volume={37},
  number={1},
  pages={26--38},
  year={1990},
  publisher={Elsevier}
}


%Why we can not extrapolate from small to large systems

@article{anderson1972mor,
  title={More is different},
  author={Anderson, Philip W},
  journal={Science},
  volume={177},
  number={4047},
  pages={393--396},
  year={1972},
  publisher={World Scientific}
}

@article{levins1966strategy,
  title={The strategy of model building in population biology},
  author={Levins, Richard},
  journal={American scientist},
  volume={54},
  number={4},
  pages={421--431},
  year={1966},
  publisher={JSTOR}
}

@article{goldenfeld1999simple,
  title={Simple lessons from complexity},
  author={Goldenfeld, Nigel and Kadanoff, Leo P},
  journal={science},
  volume={284},
  number={5411},
  pages={87--89},
  year={1999},
  publisher={American Association for the Advancement of Science}
}

%Seminal paper of May
@article{may1972will,
  title={Will a large complex system be stable?},
  author={May, Robert M},
  journal={Nature},
  volume={238},
  number={5364},
  pages={413},
  year={1972},
  publisher={Nature Publishing Group}
}

%Replica trick erklaert
@book{mezard1987spin,
  title={Spin glass theory and beyond},
  author={M{\'e}zard, Marc and Parisi, Giorgio and Virasoro, Miguel},
  year={1987},
  publisher={World Scientific Publishing Company}
}

%Review about analytical solvable random ecosystems
@article{tokita2015analytical,
  title={Analytical theory of species abundance distributions of a random community model},
  author={Tokita, Kei},
  journal={Population Ecology},
  volume={57},
  number={1},
  pages={53--62},
  year={2015},
  publisher={Springer}
}




%Perceptrons

@article{gardner1988space,
  title={The space of interactions in neural network models},
  author={Gardner, Elizabeth},
  journal={Journal of physics A: Mathematical and General},
  volume={21},
  number={1},
  pages={257},
  year={1988},
  publisher={IOP Publishing}
}


@book{engel2001statistical,
  title={Statistical mechanics of learning},
  author={Engel, Andreas and Van den Broeck, Christian},
  year={2001},
  publisher={Cambridge University Press}
}

%Farkas Lemma
@article{farkas1902theorie,
  title={Theorie der einfachen Ungleichungen.},
  author={Farkas, Julius},
  journal={Journal f{\"u}r die reine und angewandte Mathematik},
  volume={124},
  pages={1--27},
  year={1902}
}


%Sparse unique solutions of underdetermined linear equation systems
@article{wang2011unique,
  title={A unique “nonnegative” solution to an underdetermined system: From vectors to matrices},
  author={Wang, Meng and Xu, Weiyu and Tang, Ao},
  journal={IEEE Transactions on Signal Processing},
  volume={59},
  number={3},
  pages={1007--1016},
  year={2011},
  publisher={IEEE}
}

@article{donoho2005sparse,
  title={Sparse nonnegative solution of underdetermined linear equations by linear programming},
  author={Donoho, David L and Tanner, Jared},
  journal={Proceedings of the National Academy of Sciences of the U.S.A.},
  volume={102},
  number={27},
  pages={9446--9451},
  year={2005},
  publisher={National Acad Sciences}
}

%Metaorganism

@article{bosch2011metaorganisms,
  title={Metaorganisms as the new frontier},
  author={Bosch, Thomas CG and McFall-Ngai, Margaret J},
  journal={Zoology},
  volume={114},
  number={4},
  pages={185--190},
  year={2011},
  publisher={Elsevier}
}





@misc{remark, 
 	 
note={ In \cite{TM17} an additional random scatter $\epsilon x_\mu$ of these thresholds is introduced, where $x_\mu$ is a random Gaussian variable with $\left<x_\mu \right>=0$, $\left<x_\mu^2 \right>=1$ and $\epsilon$ is a small positive number. Since the sharp transition to the collective phase only occurs for vanishing scattering we consider the case $\epsilon \rightarrow 0^+$. For further details confer the supplement.}

}
  
% In \cite{TM17} an additional random scatter of these thresholds is introduced. Since the sharp transition 
%	to the collective phase occurs only in the absence of this scatter we do not include it here.
@misc{usedsolver,
note={We used the solver \textit{nnls} of the scipy.optimize package in Python.}

}


% The competitive exclusion principle
@article{armstrong1980competitive,
	title={Competitive exclusion},
	author={Armstrong, Robert A and McGehee, Richard},
	journal={The American Naturalist},
	volume={115},
	number={2},
	pages={151--170},
	year={1980},
	publisher={University of Chicago Press}
}

%Constraint satisfaction paper
@article{altieri2018constraint,
	title={Constraint satisfaction mechanisms for marginal stability and criticality in large ecosystems},
	author={Altieri, Ada and Franz, Silvio},
	journal={arXiv preprint arXiv:1805.06412},
	year={2018}
}


%Jamming and perceptron
@article{franz2016simplest,
	title={The simplest model of jamming},
	author={Franz, Silvio and Parisi, Giorgio},
	journal={Journal of Physics A: Mathematical and Theoretical},
	volume={49},
	number={14},
	pages={145001},
	year={2016},
	publisher={IOP Publishing}
}

@article{altieri2016jamming,
	title={The jamming transition in high dimension: an analytical study of the TAP equations and the effective thermodynamic potential},
	author={Altieri, Ada and Franz, Silvio and Parisi, Giorgio},
	journal={Journal of Statistical Mechanics: Theory and Experiment},
	volume={2016},
	number={9},
	pages={093301},
	year={2016},
	publisher={IOP Publishing}
}


@article{altieri2018higher,
	title={Higher-order corrections to the effective potential close to the jamming transition in the perceptron model},
	author={Altieri, Ada},
	journal={Physical Review E},
	volume={97},
	number={1},
	pages={012103},
	year={2018},
	publisher={APS}
}
